BioDiVinE: A Framework for Parallel Analysis of Biological Models

In this paper a novel tool BioDiVinEfor parallel analysis of biological models is presented. The tool allows analysis of biological models specified in terms of a set of chemical reactions. Chemical reactions are transformed into a system of multi-affine differential equations. BioDiVinE employs techniques for finite discrete abstraction of the continuous state space. At that level, parallel analysis algorithms based on model checking are provided. In the paper, the key tool features are described and their application is demonstrated by means of a case study.

==> eptcsdata.tex <==
\providecommand{\event}{R.J.Back, I.Petre, E. de Vink (Eds.): Computational\\
Models for Cell Processes (CompMod 2009)}
\providecommand{\volume}{6}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{31}
\providecommand{\eid}{3}
\pdfoutput=1

